Step-by-Step Mastery: Enhancing Soft Constraint Following Ability of Large Language Models

It is crucial for large language models (LLMs) to follow instructions that involve multiple constraints. However, it is an unexplored area to enhance LLMs' ability to follow soft constraints. To bridge the gap, we initially design a pipeline to construct datasets with high-quality outputs automatically. Additionally, to fully utilize the positive and negative samples generated during the data construction process, we choose Direct Preference Optimization (DPO) as the training method. Furthermore, taking into account the difficulty of soft constraints indicated by the number of constraints, we design a curriculum learning training paradigm based on the constraint quantity. We experimentally evaluate the effectiveness of our methods in improving LLMs' soft constraint following ability and analyze the factors driving the improvements.The datasets and code are publicly available at https://github.com/Rainier-rq/FollowSoftConstraint.

==> figures/radar.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.49\textwidth]{figures/files/radar_chart_llama_hsr.pdf}
\hfill
\includegraphics[width=0.49\textwidth]{figures/files/radar_chart_llama_ssr.pdf}
\caption{Average HSR and SSR results for LLaMA models across various constraint categories in FollowBench.}
\label{fig:kind_hsr_ssr}
\end{figure*}

